Quasars in the 4D Eigenvector 1 Context: A stroll down memory lane

Recently some pessimism has been expressed about our lack of progress in understanding quasars over the 50+ year since their discovery. It is worthwhile to look back at some of the progress that has been made - but still lies under the radar - perhaps because few people are working on optical/UV spectroscopy in this field. Great advances in understanding quasar phenomenology have emerged using eigenvector techniques. The 4D eigenvector 1 context provides a surrogate H-R Diagram for quasars with a source main sequence driven by Eddington ratio convolved with line-of-sight orientation. Appreciating the striking differences between quasars at opposite ends of the main sequence (so-called population A and B sources) opens the door towards a unified model of quasar physics, geometry and kinematics. We present a review of some of the progress that has been made over the past 15 years, and point out unsolved issues.

==> README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

